Learning Interestingness in Automated Mathematical Theory Formation

We take two key steps in automating the open-ended discovery of new mathematical theories, a grand challenge in artificial intelligence. First, we introduce $\emph{FERMAT}$, a reinforcement learning (RL) environment that models concept discovery and theorem-proving using a set of symbolic actions, opening up a range of RL problems relevant to theory discovery. Second, we explore a specific problem through $\emph{FERMAT}$: automatically scoring the $\emph{interestingness}$ of mathematical objects. We investigate evolutionary algorithms for synthesizing nontrivial interestingness measures. In particular, we introduce an LLM-based evolutionary algorithm that features function abstraction, leading to notable improvements in discovering elementary number theory and finite fields over hard-coded baselines. We open-source the $\emph{FERMAT}$ environment at this URL(https://github.com/trishullab/Fermat).

==> conjecturing_ex.tex <==

Hi! What're you doing looking at these tex files? Here's a fun easter egg from the beginning of this project.

Here we include an idealized version of how the mathematical discovery process might proceed. We start with the starting definition of natural numbers:

\begin{definition}
    The natural numbers $\mathbb{N}$ are the bundle:
    \begin{enumerate}
    \item \textbf{Zero element}: 0 is a natural number.
    \item \textbf{Successor function}: $S: \mathbb{N} \to \mathbb{N}$ which takes in a natural number and outputs the ``next'' natural number.
\end{enumerate}
\end{definition}

Note that the number two, for example, is $S(S(0))$. A principle which we now use is the idea of ``iterating a map''. 
\begin{definition}
    Given two natural number $n, m \in \mathbb{N}$, we define \emph{addition} to satisfy
    \begin{enumerate}
        \item $a + 0 = a$
        \item $a + S(b) = S(a + b)$
    \end{enumerate}
    Loosely, $a + b$ means iterating $S$ $b$ times on $a$.
\end{definition}

We continue to push the principle of iterating maps:
\begin{definition}
    Given two natural numbers $n,m \in \mathbb{N}$, we define \emph{multiplication} to satisfy
    \begin{enumerate}
        \item $a * 0 = 0$
        \item $a * S(b) = a * b + a$
    \end{enumerate}
    Loosely, $a * b$ means applying the addition operator $+(0, a)$ $b$ times.
\end{definition}

Pushing this principle once again yields powers, which are still quite useful, and afterwards tetration which becomes less interesting. (\emph{Note:} One can view this as the application of our map iteration rule.

Now we move onto another principle: The statement $a \times b = c$ actually induces relations between each pair of $\{a,b,c\}$. In particular, we learn that $a$ and $c$ are related by the \emph{existential} rule $\exists b, a \times b = c$ which we would call \textbf{divisibility}. This comes from generalization along one variable in the statement.

Checking the divisibility rule, we might start constructing examples. For example, appearing for every number in a supposed table for divisibility, we find that $1 * a = a$ so that $1$ divides $a$ for every example we can find. This suggests the \emph{universal quantifier} rule for forming a conjecture, namely:

\begin{conjecture}
    For all natural numbers $n \in \mathbb{N}$, $1 | n$.
\end{conjecture}
This one is perhaps not so interesting to us, but is useful for theory building. We might then morph this conjecture/theorem to a similar statement: 
\begin{conjecture}
    For all natural numbers $n \in \mathbb{N}$, $n | n$.
\end{conjecture}

Given these two conjectures, which we presumably are able to prove, we might then inspect the computed divisors of numbers. Checking the divisors we find certain numbers are consistent with the conjectures above but have no further divisors. This motivates the following definition:

\begin{definition}
    We call a natural number $n$ \emph{splarg} if its only divisors are $1$ and $n$.
\end{definition}

Of course, this is just the definition of prime numbers. Given that universal conjectures are interesting at their inception, some interestingness passes to \emph{splarg} numbers, which are instances where these conjectures hold more tightly.

An alternative method for deducing \emph{splarg} numbers can come from another rule. Given computed divisors of numbers, we can start to compute \emph{sizes} as in HR. We notice that of all our examples, only the number $1$ has only $1$ divisor. This motivates a conjecture
\begin{conjecture}
    The only number with $1$ divisor is $1$.
\end{conjecture}
which is, of course, true. A modification takes this conjecture and changes the value of the number of divisors to $2$. This lends itself towards \emph{splarg} numbers being defined.

Similarly, we might specialize the divisibility property for particular numbers. If there is a prior to small numbers, for example $2$, we yield the definition of \emph{zoobla} numbers. Next we use the \emph{negation principle}. Looking at the natural numbers, which inherently is interesting as we have provided it as a starting point, we consider \emph{negating} or complementing the \emph{zoobla} numbers. This yields the \emph{quarfoolie} (odd) numbers.

A \emph{commonality} production rule looks for commonalities among entries of data tables. For instance, looking at the computed set of prime numbers, and the divisors of all natural numbers (greater than 1), we notice there is always a prime. Using the universal production rule, we obtain the conjecture 

\begin{conjecture}
    For all $n \in \mathbb{N}$ with $n > 1$, we have that there exists a \emph{splarg} number satisfying $p | n$.
\end{conjecture}

A simple proof follows by strong induction on $n$. However, we do not remark on how one might synthesize this proof. Once the above conjecture is proven, we may begin investigating extensions of it - for instance, iterating on the divisibility definition, we find that for $n \geq 1$, there is a splarg $p$ and a natural number $k$ such that $n = pk$. Does $p | k$? This yields the \emph{maximality} production rule. Namely, we define the \emph{blozintra} number of $n$ with respect to $p$ to be the largest $i$ such that $p^i | n$. This happens to be well defined.

For each prime $p$ dividing $n$, we may notice that the blozintra number is unique, and further create a tuple/dictionary of blozintra numbers indexed by $p$. At this point we notice that this dictionary can be used for the \emph{uniqueness production rule} --- namely, that there is a unique prime/power tuple corresponding to each natural number. In particular, this is the unique factorization theorem of the natural numbers:

\begin{conjecture}
    For each $n \in \mathbb{N}$, there is a unique factorization into primes of $n$, up to reordering.
\end{conjecture}

This achieves one of the interesting results regarding the natural numbers. Here we detail another possible route of application. Given knowledge of the sum function, we produce another datatable by applying it on two known datatables. For instance, we choose to instantiate both operators with the \emph{splarg numbers}:
\[
\mathrm{splarg} + \mathrm{splarg} = \{4, 6, 8, 10, 12, \dots\}
\]
Using the commonality production rule, we find that this intersects with all but a small number (1) of \emph{zoobla} numbers. This motivates the universal production rule to obtain the following conjecture:

\begin{conjecture}
    Every \emph{zoobla} number greater than $2$ can be written as the sum of two \emph{splarg} numbers.
\end{conjecture}

which is better known as Goldbach's conjecture. Continuing this process could yield Goldbach's weaker conjecture (now proven):

\begin{conjecture}
    Every \emph{quarfoolie} number greater than $5$ can be written as the sum of three \emph{splarg} numbers.
\end{conjecture}

Similarly, relations between addition can help define subtraction, division, and properties about associativity, commutativity, and other well-known properties of the natural numbers. Towards getting other canonically interesting conjectures, we note that the process described for Goldbach's conjecture can yield the statement of Fermat's Last Theorem. First, consider the datatable of \emph{squares} of natural numbers, by judging that squaring is inherently interesting (perhaps because it has a low structure cost). Consider the data table formed by using the addition operator over all pairs in this datatable, and use the \emph{commonality} production rule. We find that there are commonalities - for instance $3^2 + 4^2 = 5^2$. Perhaps this is judged as \emph{interesting} and hence the production history of this datatable warranted further generalizations or modifications. Extending from squares to cubes yields different behavior, the ultimate datatable contains \emph{no} entries. This is surprising - as a small change yields a large behavior differential. This gives a conjecture which we allot high interestingness:

\begin{conjecture}
    For all natural numbers $x, y, z$ not 0, we have $x^3 + y^3 \neq z^3$.
\end{conjecture}

Generalizing on $3$ to $4$ and so on yields similar behavior which stands to provide a more general conjecture:

\begin{conjecture}[Fermat's Last Theorem]
    For all natural numbers $x,y,z, n$ which $n \geq 3$, we have $x^n + y^n \neq z^n$.
\end{conjecture}

Similarly, investigations into other quantities like $a^p - a$ can yield the statement of Fermat's little theorem. We also remark about creating operators based on a \emph{fold production rule}. In particular, on input $1$ and applying the successor function as part of a fold over addition, up to $n$, we obtain the function $f : n \mapsto n(n+1)/2$. Swapping out addition for multiplication yields the \emph{factorial} operator which itself can lead to theorems and conjectures.

In all these descriptions of a mathematician's operations, we do not include any \emph{proofs}. However, the proof objects themselves are valuable locations for generalization, lemma extraction, and concept synthesis. We don't target the \emph{learning-to-prove} process, but this is an important spot for future work. 

\subsection*{Sets}

The behavior of sets is somewhat different. For one, there are many more examples possible for sets, so eliciting useful behavior may be less possible. The data synthesis method may be heavily biased towards this end. Ultimately, we want to avoid overfitting counterexample generation as much as possible.

In this category things we would want to be able to synthesize:
\begin{enumerate}
    \item Unions and Intersections (using predicate notation, a simple conjunction/disjuction of the ``in'' operator)
    \item Set difference, Symmetric Difference
    \item Properties relation iterated unions being intersected, for example
    \item Extensions of properties to more general cases: indexed intersections/unions
    \item Subsets \& Proper Subsets
    \item De Morgan's Laws
    \item Cardinalities of sets (this may be baked in as a production rule, potentially)
    \item Power Sets
    \item Partitions
\end{enumerate}
This is about it - using this we can get quite far into group theory, for example.


\subsection*{Group Theory}
We now start with the basic definition of a group:

\begin{definition}
A group $(G, \cdot)$ consists of:
\begin{enumerate}
    \item A set $G$.
    \item A binary operation $\cdot : G \times G \to G$.
    \item An identity element $e \in G$ such that for all $g \in G$, $e \cdot g = g \cdot e = g$.
    \item An inverse for every element: for each $g \in G$, there exists $g^{-1} \in G$ such that $g \cdot g^{-1} = g^{-1} \cdot g = e$.
    \item Associativity: for all $a, b, c \in G$, we have $(a \cdot b) \cdot c = a \cdot (b \cdot c)$.
\end{enumerate}
\end{definition}

Constructing examples here is somewhat tougher - we might aim to use a finite model constructor for these. However, it is possible a lot of conjectures can be made syntactically - just by trying to boost known relations on the naturals. Using the map iteration rule on the binary operation of the group we obtain
\begin{definition}
    Given an element $g \in G$ and a natural number $n \in \mathbb{N}$, we define \emph{exponentiation} as:
    \begin{enumerate}
        \item $g^0 = e$
        \item $g^{n+1} = g^n \cdot g$
    \end{enumerate}
\end{definition}

Supposing we have some example groups constructed, perhaps by way of exploring other conjectures, we might explore the the list of powers of each group element $g \in G$. Using the \emph{commonality principle}, we find that the identity element appears in every list, but the power differs for each element. This motivates the creation of the concept

\begin{definition}
The \emph{tionick} $n$ of an element $g \in G$ satisfies $g^n = e$.
\end{definition}

However, here we propose a new production rule, the \emph{minimality} rule. Not only do we notice that there is a common identity for each of the ``cycles'' of powers, it appears many times. We are interested in the \emph{smallest} value, and hence include this notion in a production rule.

\begin{definition}
    The \emph{order} $n$ of an element $g \in G$ satisfies $g^n = e$ and is the smallest $n > 0$ with this property.
\end{definition}

Independently, we consider the \emph{substructure} production rule, intended to produce a concept of a subgroup. In particular, a subgroup satisfies all the properties of the parent group, except restricted to a subset of the carrier set. Given the concept of a subset, and knowing that the group definition includes a carrier set, we might propose the following definition using a \emph{mutation production rule}:

\begin{definition}
Given a group $(G, \cdot)$, a subgroup $H$ consists of:
\begin{enumerate}
    \item A set $H \subset G$.
    \item A binary operation $\cdot : H \times H \to H$ which operates the same as $\cdot : G \times G \to G$
    \item An identity element $e \in H$ such that for all $h \in H$, $e \cdot h = h \cdot e = h$.
    \item An inverse for every element: for each $h \in H$, there exists $h^{-1} \in H$ such that $h \cdot h^{-1} = h^{-1} \cdot h = e$.
    \item Associativity: for all $a, b, c \in H$, we have $(a \cdot b) \cdot c = a \cdot (b \cdot c)$.
\end{enumerate}
\end{definition}

However, this gives us no examples. So we are unaware if this construction is actually useful. \textbf{Somehow,} we have code which can identify subgroups in existing groups we know about. Interestingness is assigned to this concept when we find examples, justifying that it classifies some property.

By \textbf{somehow} including the concept of functions in our exploration (perhaps as part of the sets section), we can also define group homomorphisms to study how groups relate to each other:

\begin{definition}
A \emph{group homomorphism} between two groups $(G, \cdot)$ and $(H, *)$ is a function $f : G \to H$ such that for all $a, b \in G$, 
\[ f(a \cdot b) = f(a) * f(b). \]
\end{definition}

This may be backed in as a fundamental production rule trying to identify commonalities between structures (for instance, a bijective function between sets reveals the size structure to the same for both objects). By examining properties of homomorphisms, we might consider the preimage of certain sets.

\begin{definition}
    The \emph{kernel} of a homomorphism $f : G \to H$ is $f^{-1}(0)$.
\end{definition}

Independent explorations may consider datatables of the $a \cdot b$ and $b \cdot a$ for $a, b \in G$. We might notice that for some groups, this property holds true for all elements by noticing the data tables are the same. However, for others, this is not true.

\begin{definition}
    A group is \emph{snarfalien} is for all $a, b \in G$, $a \cdot b = b \cdot a$.
\end{definition}

Because this classifies certain groups and not others, it can be an interesting concept. We can rewrite \emph{snarfalien} to state that $G = \{a : \forall b \in G, a \cdot b = b \cdot a\}$. Independently we might consider the subconstruction $\{a \in G: \forall b \in G, a \cdot b = b \cdot a\}$ and compute some examples, finding that $1$ is always in this. This leads to the universal conjecture about the center of a group. Other explorations with relations to the center and the inverses datatables also show that if an element is in the center, so is its inverse. Matching these conjectures with the subgroup definition, we find we need only one more property to establish the center is a subgroup:

\begin{conjecture}
    If $a, b$ are in the center of a group $G$, then so is $a \cdot b$.
\end{conjecture}

The prover easily discharges this goal, and we have formed the theorem that the center is a subgroup!

We may now manipulate the quantity of instruct to $a \cdot b \cdot a^{-1} = b$, and consider the operation of $a \cdot . \cdot a^{-1}$. Applying this to all elements in a subgroup, we might inspect whether this yields a subgroup, and if the subgroup is the same. This can motivate the definition of normal subgroups. Further checking may yield

\begin{conjecture}
The \emph{kernel} of a group homomorphism $f : G \to H$ is a normal subgroup of $G$.
\end{conjecture}

We may also generalize the operation of taking quotients, leading to the definition of quotient groups and another interesting conjecture:

\begin{conjecture}
If $N$ is a normal subgroup of $G$, then $G/N$ is a group.
\end{conjecture}

Continuing this process can lead to well-known results such as Lagrange's theorem:

\begin{conjecture}[Lagrange's Theorem]
    If $G$ is a finite group and $H$ is a subgroup of $G$, then the order of $H$ divides the order of $G$.
\end{conjecture}
